Variable-Based Fault Localization via Enhanced Decision Tree

Fault localization, aiming at localizing the root cause of the bug under repair, has been a longstanding research topic. Although many approaches have been proposed in the last decades, most of the existing studies work at coarse-grained statement or method levels with very limited insights about how to repair the bug (granularity problem), but few studies target the finer-grained fault localization. In this paper, we target the granularity problem and propose a novel finer-grained variable-level fault localization technique. Specifically, we design a program-dependency-enhanced decision tree model to boost the identification of fault-relevant variables via discriminating failed and passed test cases based on the variable values. To evaluate the effectiveness of our approach, we have implemented it in a tool called VARDT and conducted an extensive study over the Defects4J benchmark. The results show that VARDT outperforms the state-of-the-art fault localization approaches with at least 247.8% improvements in terms of bugs located at Top-1, and the average improvements are 330.5%. Besides, to investigate whether our finer-grained fault localization result can further improve the effectiveness of downstream APR techniques, we have adapted VARDT to the application of patch filtering, where VARDT outperforms the state-of-the-art PATCH-SIM by filtering 26.0% more incorrect patches. The results demonstrate the effectiveness of our approach and it also provides a new way of thinking for improving automatic program repair techniques.

==> code/output.tex <==
\begin{lstlisting}[style=java, numbers=none,label=lst:output-comp,caption=Expected and failing test output.]
	<@\lin{1}@>  // expected output
	<@\lin{2}@>  "  -p,--period <PERIOD>  PERIOD is time duration of
	<@\lin{3}@>                          form DATE[-DATE] where DATE
	<@\lin{4}@>                          has form YYYY[MM[DD]]"
	<@\lin{5}@>  // failing test output
	<@\lin{6}@>  "  -p,--period <PERIOD>  PERIOD is time duration of
	<@\lin{7}@>                          form DATE[-DATE] where DATE has form YYYY[MM[DD]]"              //miss the second wrap point
\end{lstlisting}

==> results/ablation-mfrmar-figure.tex <==
\begin{figure}[]
	\centering
	\includegraphics[width=0.98\columnwidth]{fig/mfrmar.png}
	\caption{MAR and MFR of \tool{} and its variants}
	\label{fig:ablation-mfrmar}
\end{figure}

==> results/ablation-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[]
\centering
\caption{Top-1 results of \tool{} and its variants}
\label{tab:vardt-top1}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
Project         & \tool{} & \variant{slice} & \variant{tree} & \variant{dep} \\ \midrule
Compress        & 11.11\%                          & 22.22\%                   & 22.22\%                & 0.00\%                       \\
Gson            & 42.86\%                          & 57.14\%                   & 14.29\%                & 42.86\%                      \\
Codec           & 20.00\%                          & 0.00\%                    & 10.00\%                & 10.00\%                      \\
Csv             & 20.00\%                          & 20.00\%                   & 0.00\%                 & 20.00\%                      \\
Lang            & 26.09\%                          & 21.74\%                   & 13.04\%                & 13.04\%                      \\
JacksonXml      & 25.00\%                          & 25.00\%                   & 0.00\%                 & 50.00\%                      \\
Chart           & 25.00\%                          & 33.33\%                   & 16.67\%                & 0.00\%                       \\
JacksonCore     & 6.25\%                           & 0.00\%                    & 6.25\%                 & 6.25\%                       \\
Jsop            & 16.67\%                          & 11.11\%                   & 5.56\%                 & 0.00\%                       \\
JxPath          & 12.50\%                          & 0.00\%                    & 0.00\%                 & 12.50\%                      \\
Math            & 26.09\%                          & 21.74\%                   & 13.04\%                & 26.09\%                      \\
JacksonDatabind & 32.14\%                          & 21.43\%                   & 0.00\%                 & 32.14\%                      \\
Time            & 25.00\%                          & 8.33\%                    & 33.33\%                & 25.00\%                      \\
Cli             & 37.50\%                          & 25.00\%                   & 12.50\%                & 12.50\%                      \\
Mockito         & 28.57\%                          & 28.57\%                   & 4.76\%                 & 28.57\%                      \\
\hline
\textbf{TOTAL}           & \textbf{24.02\%}                          & \textbf{19.12\%}                   & \textbf{9.80\%}                 & \textbf{18.14\%}                      \\ \bottomrule
\end{tabular}%
}
\end{table}

\begin{table}[]
\centering
\caption{MAR results of \tool{} and its variants}
\label{tab:vardt-mar}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
Project         & \tool{} & \variant{slice} & \variant{tree} & \variant{dep} \\ \midrule
Compress        & 14.86 & 27.41        & 25.75       & 15.38      \\
Gson            & 7.24  & 16.35        & 25.26       & 7.13       \\
Codec           & 22.82 & 33.50        & 28.49       & 19.09      \\
Csv             & 8.25  & 20.75        & 31.08       & 12.58      \\
Lang            & 9.59  & 11.96        & 14.90       & 11.30      \\
JacksonXml      & 4.33  & 27.89        & 25.75       & 2.33       \\
Chart           & 6.53  & 11.28        & 18.52       & 7.36       \\
JacksonCore     & 16.69 & 26.27        & 24.97       & 16.71      \\
Jsop            & 12.41 & 27.65        & 20.81       & 15.04      \\
JxPath          & 15.64 & 22.50        & 35.60       & 17.68      \\
Math            & 12.95 & 27.95        & 22.32       & 11.62      \\
JacksonDatabind & 10.94 & 21.19        & 29.97       & 12.32      \\
Time            & 7.83  & 10.58        & 12.93       & 7.70       \\
Cli             & 5.13  & 6.81         & 25.62       & 6.43       \\
Mockito         & 7.02  & 12.98        & 14.37       & 7.56       \\
\hline
\textbf{TOTAL}  & \textbf{11.23} & \textbf{20.08} & \textbf{22.49} & \textbf{11.75}
\\ \bottomrule
\end{tabular}%
}
\end{table}

\begin{table}[]
\centering
\caption{MFR results of \tool{} and its variants}
\label{tab:vardt-mfr}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
Project         & \tool{} & \variant{slice} & \variant{tree} & \variant{dep} \\ \midrule
Compress        & 11.50         & 24.13          & 18.88          & 10.64         \\
Gson            & 6.00          & 13.33          & 23.14          & 5.93          \\
Codec           & 17.35         & 26.50          & 24.60          & 14.10         \\
Csv             & 2.00          & 16.13          & 10.00          & 10.25         \\
Lang            & 6.14          & 7.46           & 9.18           & 6.08          \\
JacksonXml      & 4.33          & 13.83          & 25.75          & 2.33          \\
Chart           & 4.41          & 7.13           & 15.00          & 5.59          \\
JacksonCore     & 12.58         & 20.42          & 21.88          & 13.75         \\
Jsop            & 10.65         & 21.44          & 17.09          & 13.76         \\
JxPath          & 12.43         & 18.71          & 26.21          & 14.36         \\
Math            & 5.82          & 14.34          & 11.90          & 5.74          \\
JacksonDatabind & 8.20          & 15.94          & 25.77          & 9.94          \\
Time            & 5.13          & 7.21           & 5.13           & 5.88          \\
Cli             & 2.57          & 3.00           & 23.86          & 3.71          \\
Mockito         & 5.78          & 10.34          & 11.42          & 5.91          \\
\hline
\textbf{TOTAL}  & \textbf{7.98} & \textbf{14.28} & \textbf{17.27} & \textbf{8.71}
\\ \bottomrule
\end{tabular}%
}
\end{table}


\begin{table}[]
\centering
\caption{ExamScore results of \tool{} and its variants}
\label{tab:vardt-es}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
Project         & \tool{} & \variant{slice} & \variant{tree} & \variant{dep} \\ \midrule
Compress        & 53.80\%                 & 42.72\%          & 45.16\%       & 56.69\%             \\
Gson            & 39.63\%                 & 28.15\%          & 42.44\%       & 32.18\%             \\
Codec           & 30.73\%                 & 24.56\%          & 36.92\%       & 28.20\%             \\
Csv             & 61.43\%                 & 38.68\%          & 65.01\%       & 68.10\%             \\
Lang            & 41.52\%                 & 26.82\%          & 37.63\%       & 48.58\%             \\
JacksonXml      & 30.24\%                 & 36.02\%          & 32.20\%       & 27.87\%             \\
Chart           & 29.72\%                 & 21.46\%          & 35.88\%       & 39.79\%             \\
JacksonCore     & 50.06\%                 & 44.03\%          & 55.11\%       & 53.04\%             \\
Jsop            & 34.07\%                 & 30.09\%          & 41.98\%       & 39.46\%             \\
JxPath          & 37.77\%                 & 41.59\%          & 46.95\%       & 46.53\%             \\
Math            & 36.41\%                 & 22.78\%          & 37.09\%       & 39.11\%             \\
JacksonDatabind & 22.90\%                 & 21.44\%          & 40.20\%       & 27.20\%             \\
Time            & 17.94\%                 & 19.58\%          & 20.93\%       & 21.73\%             \\
Cli             & 22.02\%                 & 9.13\%           & 63.80\%       & 27.26\%             \\
Mockito         & 43.72\%                 & 41.01\%          & 42.44\%       & 46.69\%             \\
\hline
\textbf{TOTAL}           & \textbf{35.85\%}                 & \textbf{28.98\%}          & \textbf{41.51\%}       & \textbf{39.78\%}             \\ \bottomrule
\end{tabular}%
}
\end{table}


==> results/backup.tex <==
\begin{table*}[t]
\centering
\caption{Experimental result summary of all approaches} 
% \jj{highlight the best result in each row, instead of bolding the last row.}}
\label{tab:othertools-topn}
\resizebox{0.75\textwidth}{!}{%
\begin{tabular}{c|rrrrrrrrr}
\toprule
%\textbf{Metric} & \textbf{\tool{}} & \textbf{UniVal} & \textbf{Baah2010} & \textbf{ESP} & \textbf{NUMFL-DLRM} & \textbf{NUMFL-QRM} & \textbf{Ochiai} & \textbf{DStar(Star=2)}
 \textbf{Metric}                                                     & \textbf{\tool{}}            & \textbf{UniVal}         &\textbf{Baah-2010}& \textbf{ESP}             & \textbf{NUMFL-DLRM} & \textbf{NUMFL-QRM} & \textbf{Ochiai}          & \textbf{Dstar (Star=2)} 
 \\ \midrule
\textbf{Top-1}  & \textbf{24.02\%} & 6.86\%  & 5.88\%   & 6.37\%  & 4.41\%     & 3.92\%    & 6.37\%  & 6.86\%        \\
\textbf{Top-3}  & \textbf{39.71\%} & 12.25\% & 10.29\%  & 9.80\%  & 8.82\%     & 11.76\%   & 14.22\% & 14.22\%       \\
\textbf{Top-5}  & \textbf{49.02\%} & 15.20\% & 15.20\%  & 12.25\% & 12.75\%    & 16.18\%   & 18.63\% & 18.14\%       \\
\textbf{Top-10} & \textbf{65.69\%} & 19.61\% & 18.14\%  & 15.69\% & 17.16\%    & 20.59\%   & 21.08\% & 20.59\% \\
\midrule
\textbf{MFR}  &  \textbf{7.98}  &  28.17  &  29.90  &  44.04  &  29.48  &  28.63  &  28.49   &  28.07  \\
\textbf{MAR}  &  \textbf{11.23}  &  49.27  &  53.15  &  65.63  & 52.02  &  49.46  & 52.46  &  51.39
\\ \bottomrule
\end{tabular}%
}
\end{table*}

\begin{table}[t]
\centering
\caption{Top-1 results of all approaches}
\label{tab:othertools-top1}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|rrrrrrrr}
\toprule
\textbf{Project}                                                     & \textbf{\tool{}}            & \textbf{UniVal}         & \begin{tabular}[c]{@{}l@{}}\textbf{Baah}\\ \textbf{-2010}\end{tabular} & \textbf{ESP}             & \begin{tabular}[c]{@{}l@{}}\textbf{NUMFL}\\ \textbf{-DLRM}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{NUMFL}\\ \textbf{-QRM}\end{tabular} & \textbf{Ochiai}          & \begin{tabular}[c]{@{}l@{}}\textbf{Dstar}\\ \textbf{(Star=2)}\end{tabular} \\ \midrule
Compress                                                    & \textbf{11.11\%}          & \textbf{11.11\%}         & \textbf{11.11\%}         & 0.00\%          & \textbf{11.11\%}         & 0.00\%          & \textbf{11.11\%}         & \textbf{11.11\%}         \\
Gson                                                        & \textbf{42.86\%}          & 14.29\%         & 14.29\%         & 0.00\%          & 0.00\%          & 0.00\%          & 14.29\%         & 14.29\%         \\
Codec                                                       & \textbf{20.00\%}          & 0.00\%          & 0.00\%          & 0.00\%          & 10.00\%         & 10.00\%         & 0.00\%          & 0.00\%          \\
Csv                                                         & \textbf{20.00\%}          & \textbf{20.00\%}         & \textbf{20.00\%}         & \textbf{20.00\%}         & 0.00\%          & 0.00\%          & \textbf{20.00\%}         & \textbf{20.00\%}         \\
Lang                                                        & \textbf{26.09\%}          & 13.04\%         & 4.35\%          & 17.39\%         & 8.70\%          & 4.35\%          & 0.00\%          & 0.00\%          \\
JXml  & \textbf{25.00\%}          & 0.00\%          & 0.00\%          & 0.00\%          & 0.00\%          & 0.00\%          & 0.00\%          & 0.00\%          \\
Chart                                                       & \textbf{25.00\%}          & 8.33\%          & 8.33\%          & 8.33\%          & 0.00\%          & 0.00\%          & 0.00\%          & 0.00\%          \\
JCore    & \textbf{6.25\%}           & \textbf{6.25\%}          & 0.00\%          & 0.00\%          & 0.00\%          & 0.00\%          & \textbf{6.25\%}          & \textbf{6.25\%}          \\
Jsoup                                                       & \textbf{16.67\%}          & 5.56\%          & 0.00\%          & 5.56\%          & 5.56\%          & 0.00\%          & 0.00\%          & 0.00\%          \\
JxPath                                                      & \textbf{12.50\%}          & 0.00\%          & 0.00\%          & 0.00\%          & 0.00\%          & \textbf{12.50\%}         & 0.00\%          & 0.00\%          \\
Math                                                        & \textbf{26.09\%}          & 13.04\%         & 13.04\%         & 17.39\%         & 13.04\%         & 13.04\%         & 13.04\%         & 13.04\%         \\
JDatabind & \textbf{32.14\%}          & 3.57\%          & 10.71\%         & 3.57\%          & 0.00\%          & 0.00\%          & 17.86\%         & 17.86\%         \\
Time                                                        & \textbf{25.00\%}          & 0.00\%          & 8.33\%          & 0.00\%          & 0.00\%          & 8.33\%          & 0.00\%          & 8.33\%          \\
Cli                                                         & \textbf{37.50\%}          & 12.50\%         & 0.00\%          & 12.50\%         & 12.50\%         & 12.50\%         & 0.00\%          & 0.00\%          \\
Mockito                                                     & \textbf{28.57\%}          & 0.00\%          & 0.00\%          & 0.00\%          & 0.00\%          & 0.00\%          & 4.76\%          & 4.76\%          \\
\midrule
\textbf{TOTAL}  & \textbf{24.02\%} & \textbf{6.86\%} & \textbf{5.88\%} & \textbf{6.37\%} & \textbf{4.41\%} & \textbf{3.92\%} & \textbf{6.37\%} & \textbf{6.86\%}
\\ \bottomrule
\end{tabular}%
}
\end{table}

\newcommand{\var}[1]{\textsc{DT}$_\mathrm{\textit{#1}}$}
\begin{table}[tb]
	\centering
	\caption{Experimental results in patch filtering}
	\label{tab:patchfilter}
	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{cc|rrrrr}
		\toprule
		\textbf{Project} & \textbf{\#All(Correct)} & \textbf{\var{Top-1}}           & \textbf{\var{Top-3}}           & \textbf{\var{Top-5}}         & \textbf{\var{Top-10}}          & \textbf{PATCH-SIM}   \\ \midrule
		Math     & 24(3)                                & 22(2)            & 22(2)            & 20(1)            & 14(0)            & 15(0)   \\
		Lang    & 10(2)                                 & 10(2)            & 10(2)            & 10(2)            & 9(1)             & 2(0)   \\
		Chart   & 14(2)                               & 14(2)            & 8(1)             & 7(1)             & 6(1)             & 4(0) \\
		Time  &  8(1)                               & 7(1)             & 6(0)             & 6(0)             & 6(0)             & 6(0)   \\
		Mockito  & 2(1)                                & 1(0)             & 1(0)             & 1(0)             & 1(0)             & -    \\ \midrule
		\textbf{TOTAL}  &58(9)& \textbf{54(7)}   & \textbf{47(5)}   & \textbf{44(4)}   & \textbf{36(2)}   & \textbf{27(0)}  \\ \midrule
		% percentage of filtered incorrect patch over all filtered patches
		\multicolumn{2}{c|}{\textbf{Precision}} & \textbf{87.04\%} & \textbf{89.36\%} & \textbf{90.90\%} & \textbf{94.44\%} & \textbf{100.00\%}   \\
		% percentage of filtered incorrect patch over all incorrect patches
		\multicolumn{2}{c|}{\textbf{Recall}} & \textbf{95.92\%} & \textbf{85.71\%} &  \textbf{81.63\%} &  \textbf{69.40\%} & \textbf{55.10\%}    \\
		\bottomrule
		% % patch accuracy after filtering
		% \textbf{Accuracy$_{patchset}$}  & \multicolumn{4}{c}{7 / (15+7) = \textbf{31.80\%}}                              & 9 / (22+9) = \textbf{29.00\%} \\ \bottomrule
	\end{tabular}%
}
\end{table}

==> results/methodscore.tex <==
\begin{table}[]
\centering
\caption{Effects of method correctness in \tool{}}
\label{tab:methodscore}
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{Metric}    & \textbf{\tool{}} & \textbf{\variant{mk}} & \textbf{\variant{ms}} \\ \midrule
\textbf{Top-1}     & 24.02\%                          & 37.75\%                & 11.76\%                       \\
\textbf{Top-3}     & 39.71\%                          & 63.73\%                & 27.45\%                       \\
\textbf{Top-5}     & 49.02\%                          & 71.08\%                & 39.71\%                       \\
\textbf{Top-10}    & 65.69\%                          & 80.39\%                & 57.35\%                       \\
\textbf{MAR}       & 11.23                            & 4.67                   & 14.33                         \\
\textbf{MFR}       & 7.98                             & 3.10                   & 10.26                         \\
\textbf{ExamScore} & 35.85\%                          & 54.76\%                & 43.83\%                       \\ \bottomrule
\end{tabular}
\end{table}

==> results/otherTools-figure.tex <==
\begin{figure}[]
	\centering
	\includegraphics[width=0.95\columnwidth]{fig/baselinemfr.png}
	\caption{MAR and MFR of \tool{} and baseline approaches}
	\label{fig:othertools}
\end{figure}





==> results/slicingEffect-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\caption{Performance of \tool{}}
\label{tab:performance-vardt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|cccc}
\toprule
\textbf{Project} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Reduced percentage\\ by slicing\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Ratio to\\ the searching space\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Time cost of\\ tree generation (ms)\end{tabular}} \\ \midrule
Compress       & 33.93\%          & 4.04\%          & 274           \\
Gson           & 37.35\%          & 4.54\%          & 709           \\
Codec          & 37.18\%          & 2.13\%          & 567           \\
Csv            & 18.61\%          & 1.98\%          & 341           \\
Lang           & 18.62\%          & 5.11\%          & 294           \\
JXml           & 42.86\%          & 1.94\%          & 1460          \\
Chart          & 24.13\%          & 4.87\%          & 355           \\
JCore          & 38.96\%          & 4.53\%          & 4469          \\
Jsoup          & 41.99\%          & 3.61\%          & 3944          \\
JxPath         & 27.17\%          & 2.83\%          & 3344          \\
Math           & 42.19\%          & 6.57\%          & 534           \\
JDatabind      & 39.01\%          & 2.71\%          & 6866          \\
Time           & 18.45\%          & 4.48\%          & 1228          \\
Cli            & 27.33\%          & 3.93\%          & 3478          \\
Mockito        & 31.06\%          & 8.08\%          & 1250          \\
\hline
\textbf{Total} & \textbf{31.92\%} & \textbf{4.09\%} & \textbf{1941} \\ \bottomrule
\end{tabular}
}
\end{table}
